TopoNav: Topological Navigation for Efficient Exploration in Sparse Reward Environments

Autonomous robots exploring unknown environments face a significant challenge: navigating effectively without prior maps and with limited external feedback. This challenge intensifies in sparse reward environments, where traditional exploration techniques often fail. In this paper, we present TopoNav, a novel topological navigation framework that integrates active mapping, hierarchical reinforcement learning, and intrinsic motivation to enable efficient goal-oriented exploration and navigation in sparse-reward settings. TopoNav dynamically constructs a topological map of the environment, capturing key locations and pathways. A two-level hierarchical policy architecture, comprising a high-level graph traversal policy and low-level motion control policies, enables effective navigation and obstacle avoidance while maintaining focus on the overall goal. Additionally, TopoNav incorporates intrinsic motivation to guide exploration toward relevant regions and frontier nodes in the topological map, addressing the challenges of sparse extrinsic rewards. We evaluate TopoNav both in the simulated and real-world off-road environments using a Clearpath Jackal robot, across three challenging navigation scenarios: goal-reaching, feature-based navigation, and navigation in complex terrains. We observe an increase in exploration coverage by 7- 20%, in success rates by 9-19%, and reductions in navigation times by 15-36% across various scenarios, compared to state-of-the-art methods

==> Sections/draft.tex <==
\section{Draft}

% \section{Revisions and Clarifications}

% In response to the feedback received, we have made several revisions to enhance the clarity, detail, and reproducibility of our proposed method. 

% \subsection{Topological Map Creation}
% We have clarified the process of topological map creation in the revised Section~\ref{sec:topomap_creation}, providing a step-by-step description of the algorithm and ensuring consistency in the definitions. This includes a detailed account of how nodes and edges are added to the map, the criteria for node expansion, and the mechanism by which the map informs the agent's navigation strategy.

% \subsection{Intrinsic Rewards}
% The revised Section~\ref{sec:intrinsic_rewards} now includes a comprehensive explanation of the intrinsic reward system. We have disclosed the specific weight coefficients used for each reward function, along with the methodology employed to determine these values. Furthermore, we have included a supplementary document as part of the supplementary material, which outlines the hyperparameter tuning process and the empirical evaluations that led to the selection of these coefficients, ensuring reproducibility.

% \subsection{Strengthened Evaluation}
% Acknowledging the need for a robust evaluation, we have expanded our comparison in Section~\ref{sec:evaluation}. The revised evaluation now includes baseline methods that employ intrinsic rewards and additional information sources for a fair and direct comparison. Moreover, we have conducted an ablation study, presented in Section~\ref{sec:ablation_study}, which isolates the impact of topological subgoals and the individual intrinsic reward functions. This study aims to quantify the contribution of each component to the overall performance of \textit{TopoNav}.

% \section{Conclusion and Future Work}

% With these amendments, the paper now provides a more rigorous and detailed exposition of \textit{TopoNav}, its mechanisms, and its evaluation. We believe that these enhancements have addressed the concerns raised and have strengthened the contributions of our work. Future work will aim to explore the scalability of the method in more diverse and challenging real-world scenarios and to experiment with alternative intrinsic reward strategies that could further improve the system's performance.


% \section{Revised Intrinsic Rewards Methodology}

% In the revised manuscript, we have amended the section on intrinsic rewards to acknowledge the foundational work that has informed our approach. Each intrinsic reward function utilized in \textit{TopoNav} is now accompanied by citations to the original methods from which they are derived or inspired.

% Specifically, the Information Gain reward function, integral to our method, builds upon the principles of potential-based reward shaping. As such, we have clarified that the scaling factor $\gamma$ is not arbitrary but corresponds to the discount factor used in the external reward function, aligning with the established framework in the literature. This connection is now explicitly stated, and the seminal papers on potential-based reward shaping have been cited to ensure proper attribution and to aid in reproducibility.

% The revised section reads as follows:

% \subsection{Information Gain Intrinsic Reward}
% The Information Gain reward, an intrinsic motivation in \textit{TopoNav}, is formulated based on the concept of potential-based reward shaping. This approach enhances the agent's learning process by incorporating a measure of novelty or uncertainty reduction with each observed state. The discount factor $\gamma$, inherited from the external reward function, ensures temporal consistency and theoretically guarantees policy invariance. Following the foundational work by Ng et al. [reference to original paper], we define the Information Gain reward as follows:

% \begin{equation}
% R_{\text{info}}(s, s') = \gamma (V(s') - V(s)),
% \end{equation}

% where $V(s)$ denotes the potential of state $s$, capturing the anticipated future information gain from visiting state $s$.

% \section{Conclusion}
% These revisions provide a clearer understanding of the intrinsic reward functions within \textit{TopoNav} and their theoretical underpinnings. By explicitly referencing the influential research that underlies our approach, we aim to enhance the clarity and academic rigor of our work.
% %




Baselines to consider:

HTMap: Hierarchical Topological Mapping

TopoMap

Graph-based Topological Exploration Planning in Large-scale 3D
Environments

Active Neural Topological Mapping for Multi-Agent Exploration

PlaceNav: Topological Navigation through Place Recognition
Neural Topological SLAM for Visual Navigation
ViNG: Learning Open-World Navigation with Visual Goals
Lifelong Topological Visual Navigation
Semi-parametric Topological Memory for Navigation
Topomap: Topological Mapping and Navigation Based on Visual SLAM Maps


\section{Methodology}

\subsection{Topological Map Representation}
TopoNav represents the environment topology as an undirected graph $\mathcal{G} = (\mathcal{N}, \mathcal{E})$, where $\mathcal{N}$ is the set of nodes and $\mathcal{E}$ denotes the set of edges. Each node $n \in \mathcal{N}$ encodes the 3D position $\vec{p}n \in \mathbb{R}^3$, a feature descriptor $\phi_n$ capturing local geometry and semantics, and an exploration status $\xi_n \in {0, 1}$ indicating if the node has been visited. Edges $e = (n_i, n_j) \in \mathcal{E}$ represent feasible paths between connected nodes $n_i, n_j \in \mathcal{N}$, storing traversal cost $c{ij}$ and obstacle information $\mathcal{O}_{ij}$.

As the robot explores, the graph $\mathcal{G}$ is updated based on the robot's pose estimate $\vec{x}_t \in \mathbb{R}^6$ and sensor observations $\mathcal{Z}_t$ at time $t$. From the sensor data $\mathcal{Z}_t$ (e.g., LiDAR point cloud), we extract a set of environmental features $\mathcal{F}_t = {f_1, f_2, \ldots, f_m}$ via a segmentation function $\Phi$:
\begin{equation}
\mathcal{F}_t = \Phi(\mathcal{Z}_t)
\end{equation}

Each feature $f_i \in \mathcal{F}t$ is matched to the closest node $n^* \in \mathcal{N}$ based on descriptor distance $d(\phi{n^}, \phi_{f_i})$. If the minimum distance exceeds a threshold $\tau_n$, a new node $n^{new}$ is instantiated with $\vec{p}{n^{new}} = \vec{x}t$, $\phi{n^{new}} = \phi*{f_i}$, and $\xi_{n^{new}} = 1$. Additionally, an edge $e^{new} = (n^, n^{new})$ is formed with $c_{e^{new}} = |\vec{p}_{n^} - \vec{x}_t|2$ and $\mathcal{O}{e^{new}} = \text{ObstacleInfo}(\mathcal{Z}_t, \vec{x}t, \vec{p}{n^*})$, where $\text{ObstacleInfo}$ processes the sensor data to detect obstacles along the path $(\vec{x}t, \vec{p}{n^*})$.

\subsection{Hierarchical Reinforcement Learning}
We model TopoNav's navigation task as a hierarchical Markov Decision Process (HMDP) $\langle \mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \rho \rangle$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ the action space, $\mathcal{P}$ the transition dynamics, $\mathcal{R}$ the reward function, and $\rho$ the hierarchical policy that maps states to actions $a = \rho(s)$.

The hierarchical policy $\rho$ comprises two components: a meta-policy $\rho^M$ that selects the next sub-goal or node $g^* \in \mathcal{N}$ from the topological map to navigate towards, and a lower-level policy $\rho^L$ determining the robot's primitive actions $a_t$ for reaching $g^$ while respecting local constraints like obstacles.
\begin{align}
g^ &= \rho^M(s_t, \mathcal{G}) \
a_t &= \rho^L(s_t, g^*)
\end{align}

We optimize $\rho^M$ and $\rho^L$ to maximize the following joint reward objective, balancing extrinsic goal-reaching rewards $\mathcal{R}^{ext}$ with intrinsic curiosity rewards $\mathcal{R}^{int}$ for exploration:
\begin{equation}
\label{eq:obj}
\max_{\rho^M, \rho^L} \mathbb{E}{\substack{\tau \sim \rho^M, \rho^L \ s_t, a_t \sim \tau}} \left[ \sum{t=0}^\infty \gamma^t \left( \mathcal{R}^{ext}(s_t, a_t, s_{t+1}) + \mathcal{R}^{int}(s_t, a_t, s_{t+1}) \right) \right]
\end{equation}
where $\tau$ denotes the trajectory induced by $\rho^M, \rho^L$, and $\gamma \in [0, 1)$ is the discount factor.

The learning process alternates between meta-policy optimization for high-level navigation objectives, and low-level policy optimization for local control based on the current sub-goal $g^*$. We employ Proximal Policy Optimization (PPO) to learn each policy component, leveraging the hierarchical structure for improved sample efficiency.

% \begin{algorithm}[h]
% \caption{TopoNav Training Procedure}
% \begin{algorithmic}
% \STATE Initialize $\rho^M, \rho^L$ with random weights $\theta^M, \theta^L$
% \FOR{iteration $= 1, \ldots, N$}
% \STATE Sample trajectories $\tau_i \sim \pi_{\theta^M}, \pi_{\theta^L}$
% \STATE Optimize $\theta^M$ on trajectories $\tau_i$ using PPO \
% \hspace*{1em} with reward $\mathcal{R}^{ext} + \mathcal{R}^{int}$
% \FOR{trajectory $\tau_i$}
% \FOR{$t = 1, \ldots, T_i$}
% \STATE $g^t \gets \rho^M{\theta^M}(s_t, \mathcal{G})$
% \STATE Collect sub-trajectory $\tau^L_t$ for $g^_t$
% \STATE Optimize $\theta^L$ on $\tau^L_t$ using PPO  \
% \hspace*{1em}with reward $\mathcal{R}^{ext} + \mathcal{R}^{int}$
% \ENDFOR
% \ENDFOR
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

\subsection{Intrinsic Curiosity Rewards}
TopoNav employs an intrinsic reward signal $\mathcal{R}^{int}$ based on novelty, information gain, and curiosity to incentivize exploring new areas when extrinsic rewards are sparse:

\begin{align}
    \mathcal{R}^{int}(s_t, a_t, s_{t+1}) &= \lambda_1 \cdot \textbf{1}{\text{unvisited}}(s{t+1}) + \lambda_2 \cdot \textbf{I}\text{gain}(s{t+1} | s_t, \mathcal{G}) \
    &\quad + \lambda_3 \cdot \textbf{1}\text{subgoal} (s{t+1}) + \lambda_4 \cdot d(s_{t+1}, \mathcal{G})
\end{align}

The first term rewards visiting unvisited states $s_{t+1}$ with previously unseen features $\phi_{s_{t+1}}$. $\textbf{I}\text{gain}$ computes the information gain of transitioning to $s{t+1}$ given the current map $\mathcal{G}$, incentivizing exploratory actions that reduce uncertainty. The third term provides a bonus for reaching the current sub-goal encoded within $\mathcal{G}$. Finally, $d(s_{t+1}, \mathcal{G})$ is a distance-based heuristic encouraging the robot to navigate towards unexplored regions far from the existing map's coverage.

This intrinsic motivation coupled with the hierarchical decomposition enables TopoNav to pursue promising areas for expanding its knowledge of the environment topology through a series of intermediate sub-goals, while still making progress towards the high-level navigation objective defined by $\mathcal{R}^{ext}$.


-------------------------------------------

% \begin{algorithm}[h]
% \caption{Active Topological Mapping within HRL}
% \label{alg:mapping_hrl}
% \begin{algorithmic}[1]
% \REQUIRE Topological map $\mathcal{G} = (\mathcal{N}, \mathcal{E})$, sensor data $\mathcal{Z}t$, pose estimate $\vec{x}t$, meta-policy $\rho^M$, low-level policy $\rho^L$
% \STATE Extract environmental features $\mathcal{F}t = \Phi(\mathcal{Z}t)$
% \FOR{feature $f_i \in \mathcal{F}t$}
% \STATE Find closest node $n^* = \argmin{n \in \mathcal{N}} d(\phi_n, \phi{f_i})$
% \IF{$d(\phi{n^*}, \phi{f_i}) > \tau_n$}
% \STATE Instantiate new node $n^{new}$ with:
% \STATE $\vec{p}{n^{new}} = \vec{x}t$, $\phi{n^{new}} = \phi_{f_i}$, $\xi_{n^{new}} = 1$
% \STATE $\mathcal{N} \gets \mathcal{N} \cup {n^{new}}$
% \STATE Form new edge $e^{new} = (n^, n^{new})$ with:
% \STATE $c_{e^{new}} = |\vec{p}_{n^} - \vec{x}_t|2$
% \STATE $\mathcal{O}{e^{new}} = \text{ObstacleInfo}(\mathcal{Z}_t, \vec{x}t, \vec{p}{n^})$
% \STATE $\mathcal{E} \gets \mathcal{E} \cup {e^{new}}$
% \ENDIF
% \ENDFOR
% \STATE Select subgoal $g^ = \rho^M(s_t, \mathcal{G})$ using meta-policy
% \STATE Reach $g^$ by executing low-level actions $a_t = \rho^L(s_t, g^)$
% \STATE \textbf{return} Updated topological map $\mathcal{G}$
% \end{algorithmic}
% \end{algorithm}

% In Algorithm~\ref{alg:mapping_hrl}, after updating the topological map $\mathcal{G}$ based on new sensor observations, the meta-policy $\rho^M$ is used to select the next subgoal $g^$ to navigate towards. The low-level policy $\rho^L$ then generates actions $a_t$ to reach $g^$ while considering local constraints. This integrates the mapping process with the hierarchical policies being learned.

% \begin{algorithm}[h]
% \caption{Hierarchical Objective Selection in HRL}
% \label{alg:selection_hrl}
% \begin{algorithmic}[1]
% \REQUIRE Current state $s_t$, objective set $\mathcal{O} = {o_1, o_2, \ldots, o_n}$, meta-policy $\rho^M$
% \STATE Evaluate meta-policy $\rho^M(s_t, o_i)$ for each objective $o_i \in \mathcal{O}$
% \STATE Select objective $o^* = \argmax_{o_i \in \mathcal{O}} \rho^M(s_t, o_i)$
% \STATE \textbf{return} Selected objective $o^*$
% \end{algorithmic}
% \end{algorithm}

% Algorithm~\ref{alg:selection_hrl} replaces the previous objective prioritization scheme with a direct selection using the meta-policy $\rho^M$. The meta-policy is evaluated for each objective $o_i$ in the current state $s_t$, and the objective $o^*$ with the highest policy value is chosen. This aligns the objective selection with the learned HRL policies.

% \begin{algorithm}[h]
% \caption{HRL-based Topological Navigation}
% \label{alg:navigation_hrl}
% \begin{algorithmic}[1]
% \REQUIRE Topological map $\mathcal{G}$, global navigation goal $g_G$, meta-policy $\rho^M$, low-level policy $\rho^L$
% \WHILE{$g_G$ not reached}
% \STATE $s_t \gets$ GetCurrentState()
% \STATE $\mathcal{G} \gets$ UpdateMap($\mathcal{G}, s_t$) via Algorithm~\ref{alg:mapping_hrl}
% \STATE $o^* \gets$ SelectObjective($s_t, \mathcal{G}, \rho^M$) via Algorithm~\ref{alg:selection_hrl}
% \WHILE{$o^$ not completed}
% \STATE Select subgoal $g^ = \rho^M(s_t, \mathcal{G}, o^)$
% \STATE Reach $g^$ by executing low-level actions $a_t = \rho^L(s_t, g^*)$
% \STATE Update state $s_t$ based on action outcomes
% \ENDWHILE
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}

% Algorithm~\ref{alg:navigation_hrl} outlines the overall HRL-based topological navigation process. The robot alternates between updating the topological map $\mathcal{G}$ using Algorithm~\ref{alg:mapping_hrl}, selecting high-level navigation objectives $o^$ using Algorithm~\ref{alg:selection_hrl} with the meta-policy $\rho^M$, and reaching subgoals $g^$ chosen by $\rho^M$ using low-level actions from $\rho^L$. This continues until the global goal $g_G$ is reached.



-----


% \begin{algorithm}[!htb]
% \DontPrintSemicolon
% \caption{TopoNav: Topological Map Generation and Navigation with h-DQN}
% \label{alg:toponav}
% \KwIn{$G_g$, the global end goal for navigation}
% \KwOut{$T_m$, the topological map with nodes ($N$) and edges ($E$)}
% \BlankLine
% Initialize meta-controller $Q^{\mu}(s, g; \theta^{\mu})$ and sub-controllers $Q^{g}(s, a; \theta^{g})$;
% Initialize replay buffers $\mathcal{D}^{\mu}$ and $\mathcal{D}^{g}$ for each subgoal $g$;
% $T_m \gets \emptyset$;
% $s_0 \gets \text{GetInitialState()}$;
% $g_0 \gets G_g$;
% \For{each step $t$}{
% $\mathcal{L} \gets \text{DetectLandmarks}(s_t)$;
% \For{each landmark $l \in \mathcal{L}$}{
% \If{$\max_{v \in \mathcal{V}} \text{sim}(\mathbf{x}l, \mathbf{x}v) < \tau$}{
% Add $l$ as a new node to $T_m$ and update edges;
% Set $g_t$ to the new subgoal $l$;
% Break;
% }
% }
% \eIf{$g_t$ is not $G_g$}{
% Select action $a_t$ using $Q^{g_t}(s_t, a; \theta^{g_t})$ with exploration;
% Execute action $a_t$ and observe new state $s{t+1}$ and reward $r_t$;
% $r_t \gets \text{CalculateReward}(s_t, s{t+1}, g_t, G_g)$ (Algorithm \ref{alg:toponav_reward});
% Store transition $(s_t, g_t, a_t, r_t, s_{t+1})$ in $\mathcal{D}^{g_t}$;
% Update $Q^{g_t}(s, a; \theta^{g_t})$ using stored transitions in $\mathcal{D}^{g_t}$;
% \If{$s_{t+1}$ is the selected subgoal $g_t$}{
% Set $g_t$ to $G_g$;
% }
% }{
% Select subgoal $g_t$ using $Q^{\mu}(s_t, g; \theta^{\mu})$ with exploration;
% Store transition $(s_t, g_t, r_t, s_{t+1})$ in $\mathcal{D}^{\mu}$;
% Update $Q^{\mu}(s, g; \theta^{\mu})$ using stored transitions in $\mathcal{D}^{\mu}$;
% }
% $s_t \gets s_{t+1}$;
% }
% \Return{$T_m$};
% \end{algorithm}



\begin{algorithm}
\DontPrintSemicolon % Disables semicolons at the end of each line
\caption{TopoNav: Topological Map Generation and Navigation}
\label{alg:toponav}
\KwIn{$G_g$, the global end goal for navigation}
\KwIn{$d_\text{thresh}$, the distance threshold for subgoal generation}
\KwOut{$T_m$, the topological map with nodes ($N$) and edges ($E$)}
\BlankLine
Initialize meta-controller $Q^\mu(s, g; \theta^\mu)$ and sub-controllers $Q^g(s, a; \theta^g)$.\;
Initialize replay buffers $\mathcal{D}^\mu$ and $\mathcal{D}^g$ for each subgoal $g$.\;
$T_m \leftarrow \emptyset$.\;
$s_0 \leftarrow \text{GetInitialState()}$.\;
$g_0 \leftarrow G_g$.\;
\For{each step $t$}{
    $\mathcal{L} \leftarrow \text{DetectLandmarks}(s_t)$.\;
    \eIf{\text{len}($\mathcal{L}$) == 0 \textbf{and} $\text{dist}(s_t, g_t) > d_\text{thresh}$}{
        Generate new subgoal $g'$ along the trajectory towards $G_g$ at distance $d_\text{thresh}$.\;
        Add $g'$ as a new node to $T_m$ and update edges.\;
        Set $g_t$ to the new subgoal $g'$.\;
    }{
        \For{each landmark $l \in \mathcal{L}$}{
            \If{$\max_{v \in \mathcal{V}} \text{sim}(\mathbf{x}_l, \mathbf{x}_v) < \tau$}{
                Add $l$ as a new node to $T_m$ and update edges.\;
                Set $g_t$ to the new subgoal $l$.\;
                \textbf{break}\;
            }
        }
    }
    \eIf{$g_t$ is not $G_g$}{
        Select action $a_t$ using $Q^{g_t}(s_t, a; \theta^{g_t})$ with exploration.\;
        Execute action $a_t$ and observe new state $s_{t+1}$ and reward $r_t$.\;
        $r_t \leftarrow \text{Calculate Reward} ( Equation ~\ref{reward})$.\;
        Store transition $(s_t, g_t, a_t, r_t, s_{t+1})$ in $\mathcal{D}^{g_t}$.\;
        Update $Q^{g_t}(s, a; \theta^{g_t})$ using stored transitions in $\mathcal{D}^{g_t}$.\;
        \If{$s_{t+1}$ is the selected subgoal $g_t$}{
            Set $g_t$ to $G_g$.\;
        }
    }{
        Select subgoal $g_t$ using $Q^\mu(s_t, g; \theta^\mu)$ with exploration.\;
        Store transition $(s_t, g_t, r_t, s_{t+1})$ in $\mathcal{D}^\mu$.\;
        Update $Q^\mu(s, g; \theta^\mu)$ using stored transitions in $\mathcal{D}^\mu$.\;
    }
    $s_t \leftarrow s_{t+1}$.\;
}
\Return{$T_m$}\;
\end{algorithm}

----------------------------------------------

% \textbf{Theorem 1 (Subgoal Reachability):} Given a topological map $G = (V, E)$ constructed by TopoNav, where $V$ is the set of nodes (subgoals) and $E$ is the set of edges (navigable paths), for any two nodes $v_i, v_j \in V$, if there exists a path from $v_i$ to $v_j$ in $G$, then the sub-controller policy $\pi_s$ learned by TopoNav can navigate the robot from $v_i$ to $v_j$ with a probability of at least $1 - \epsilon$, where $\epsilon$ is a small positive constant.

% Proof: Let $P_{ij} = {v_i, e_{i1}, v_1, e_{12}, v_2, \dots, e_{(k-1)j}, v_j}$ be a path from node $v_i$ to node $v_j$ in the topological map $G$, where $e_{pq} \in E$ represents the edge connecting nodes $v_p$ and $v_q$.

% For each edge $e_{pq}$ in the path $P_{ij}$, the sub-controller policy $\pi_s$ learns to navigate from node $v_p$ to node $v_q$ by maximizing the expected cumulative reward. 
% According to the convergence guarantee of the DQN algorithm [19], the Q-values of the sub-controller policy converge to the optimal values $Q^*(s, a)$ in the limit of infinite training iterations, under the assumptions of adequate exploration and a suitable learning rate schedule.

% The optimal Q-values satisfy the Bellman optimality equation:
% $$Q^(s, a) = \mathbb{E}[R(s, a) + \gamma \max_{a'} Q^(s', a')]$$
% where $s$ is the current state, $a$ is the action, $R(s, a)$ is the reward function, $\gamma$ is the discount factor, and $s'$ is the next state.

% Given the convergence of the Q-values to their optimal values, the sub-controller policy $\pi_s$ selects actions that maximize the expected cumulative reward for each edge traversal. Thus, for each edge $e_{pq}$ in the path $P_{ij}$, the probability of successfully navigating from node $v_p$ to node $v_q$ using the learned sub-controller policy $\pi_s$ is at least $1 - \epsilon_{pq}$, where $\epsilon_{pq}$ is a small positive constant.

% Applying the chain rule of probability, the probability of successfully navigating from node $v_i$ to node $v_j$ along the path $P_{ij}$ using the sub-controller policy $\pi_s$ is at least:
% $$(1 - \epsilon_{i1})(1 - \epsilon_{12})\dots(1 - \epsilon_{(k-1)j}) \geq (1 - \max_{p,q} \epsilon_{pq})^k \geq 1 - k \max_{p,q} \epsilon_{pq}$$

% By setting $\epsilon = k \max_{p,q} \epsilon_{pq}$, we can conclude that the sub-controller policy $\pi_s$ learned by TopoNav can navigate the robot from node $v_i$ to node $v_j$ with a probability of at least $1 - \epsilon$, given the existence of a path $P_{ij}$ in the topological map $G$. $\square$



\section{Theoretical Foundations}

\subsection{Subgoal Reachability}
\textbf{Theorem 1 (Subgoal Reachability).} \textit{Given a topological map $G = (V, E)$ constructed by TopoNav, where $V$ is the set of nodes (subgoals) and $E$ is the set of edges (navigable paths), for any two nodes $v_i, v_j \in V$, if there exists a path from $v_i$ to $v_j$ in $G$, then the sub-controller policy $\pi_s$ learned by TopoNav can navigate the robot from $v_i$ to $v_j$ with a probability of at least $1 - \epsilon$, where $\epsilon$ is a small positive constant representing the upper bound of navigation failure probability, taking into account environmental stochasticity and learning algorithm convergence.}

\textbf{Proof.} Let $P_{ij} = \{v_i, e_{i1}, v_1, e_{12}, v_2, \dots, e_{(k-1)j}, v_j\}$ denote a path from node $v_i$ to node $v_j$ in the topological map $G$, with $e_{pq} \in E$ representing the edge connecting nodes $v_p$ and $v_q$, and $k$ the number of edges in the path.

Assuming adequate exploration and appropriate learning rate adjustments, the sub-controller policy $\pi_s$ learns to maximize the expected cumulative reward for traversing each edge in $P_{ij}$. Given the DQN's convergence towards optimal Q-values, the sub-controller $\pi_s$ effectively navigates across each edge $e_{pq}$ in $P_{ij}$. The probability of successful navigation from $v_p$ to $v_q$ for each edge is at least $1 - \epsilon_{pq}$, with $\epsilon_{pq}$ being a small positive constant reflecting uncertainties and algorithmic approximation errors.

For successful navigation along the entire path $P_{ij}$, the aggregated success probability, by the chain rule of probability, is:

\begin{equation}
    \prod_{\substack{all \; e_{pq} \in P_{ij}}} (1 - \epsilon_{pq}) \geq (1 - \max_{p,q} \epsilon_{pq})^k \geq 1 - k \max_{p,q} \epsilon_{pq},
\end{equation}

where $\epsilon = k \max_{p,q} \epsilon_{pq}$ encapsulates the compounded effect of individual uncertainties over the path length $k$. Thus, the sub-controller policy $\pi_s$ ensures navigation from $v_i$ to $v_j$ with at least a $1 - \epsilon$ probability, underpinning the robustness of TopoNav's path planning and execution in face of environmental and algorithmic variabilities. $\blacksquare$


\subsection{Subgoal Reachability}
\textbf{Theorem 1 (Subgoal Reachability)}. \textit{Given a topological map $G = (V, E)$ by TopoNav, for any two nodes $v_i, v_j \in V$, if a path from $v_i$ to $v_j$ exists, then the sub-controller policy $\pi_s$ can navigate from $v_i$ to $v_j$ with probability $\geq 1 - \epsilon$, where $\epsilon$ is a small positive constant.}

\textbf{Proof}. Consider a path $P_{ij} = \{v_i, \dots, v_j\}$ in $G$. The policy $\pi_s$, leveraging DQN, aims to maximize expected rewards for transitions between nodes along $P_{ij}$. By DQN's convergence, $\pi_s$ optimally selects actions for each transition, with success probability $\geq 1 - \epsilon_{pq}$ for an edge $e_{pq}$. Given $P_{ij}$ contains $k$ edges, the overall success probability from $v_i$ to $v_j$ is $\prod_{e_{pq} \in P_{ij}} (1 - \epsilon_{pq})$. Since $\epsilon_{pq}$ is small, this product is $\geq 1 - \epsilon$, where $\epsilon = k \max \epsilon_{pq}$, establishing the sub-controller's high-probability navigation capability. $\square$


\subsection{Subgoal Reachability in Hierarchical Framework}
\textbf{Theorem 1 (Subgoal Reachability)}. \textit{Given a topological map $G = (V, E)$ constructed by TopoNav using an h-DQN approach, where $V$ represents the set of nodes (subgoals) and $E$ represents the navigable paths between these nodes, for any two nodes $v_i, v_j \in V$, if there exists a path from $v_i$ to $v_j$ in $G$, the hierarchical policy structure ensures that the robot can navigate from $v_i$ to $v_j$ with a probability of at least $1 - \epsilon$, where $\epsilon$ is a small positive constant.}

\textbf{Proof}. The h-DQN framework in TopoNav comprises two levels of decision-making: a high-level policy selecting subgoals, and a low-level policy determining actions to reach these subgoals. Let $P_{ij} = \{v_i, \dots, v_j\}$ denote a sequence of subgoals forming a path in $G$.

1. \textit{High-Level Convergence}: The high-level policy learns to select optimal subgoals that lead towards the final goal, leveraging the structure of $G$. Given sufficient exploration and under appropriate training conditions, this policy converges towards selecting sequences of subgoals that maximize the overall expected reward, effectively navigating the hierarchical structure of tasks.

2. \textit{Low-Level Convergence}: For each pair of successive subgoals $(v_p, v_q)$ in $P_{ij}$, the low-level policy, akin to DQN's convergence mechanism, learns to select actions that navigate the robot from $v_p$ to $v_q$. This process resembles the DQN convergence guarantee, where the policy learns to maximize expected rewards for transitions between subgoals, achieving a success probability of at least $1 - \epsilon_{pq}$ for each transition.

3. \textit{Overall Probability of Success}: Combining the high-level and low-level policies, the probability of successfully navigating from $v_i$ to $v_j$ is the product of success probabilities for each subgoal transition in $P_{ij}$. This aggregated probability is $\geq (1 - \max \epsilon_{pq})^k \geq 1 - k \max \epsilon_{pq}$, with $\epsilon = k \max \epsilon_{pq}$ encapsulating the compounded uncertainties across the path.

The theorem concludes that through the hierarchical integration of decision-making policies, TopoNav can ensure high-probability navigation between any two subgoals in the topological map, leveraging the strengths of both h-DQN's hierarchical framework and the foundational DQN convergence principles. $\square$



\section{Theoretical Foundations}

\subsection{Subgoal Reachability}
\textbf{Theorem 1 (Subgoal Reachability)}. \textit{Given a topological map $G = (V, E)$ constructed by TopoNav, with $V$ representing nodes (subgoals) and $E$ representing edges (navigable paths), for any two nodes $v_i, v_j \in V$, if a path exists from $v_i$ to $v_j$ in $G$, then the sub-controller policy $\pi_s$ learned by TopoNav can navigate the robot from $v_i$ to $v_j$ with a probability of at least $1 - \epsilon$. Here, $\epsilon$ is a small positive constant representing the upper bound of navigation failure probability, which accounts for environmental stochasticity and the convergence of the learning algorithm.}

\textbf{Proof}. Consider $P_{ij} = \{v_i, e_{i1}, v_1, e_{12}, v_2, \dots, e_{(k-1)j}, v_j\}$ as a path from node $v_i$ to node $v_j$ within the topological map $G$, where $e_{pq} \in E$ signifies an edge connecting nodes $v_p$ and $v_q$, and $k$ denotes the total number of edges along this path.

With adequate exploration and suitable learning rate adjustments, the sub-controller policy $\pi_s$, utilizing the principles of Deep Q-Network (DQN) algorithms, is trained to optimize the expected cumulative reward for each segment of $P_{ij}$. This optimization ensures that for every edge $e_{pq}$ along the path, there exists a high probability, at least $1 - \epsilon_{pq}$, of successfully navigating from $v_p$ to $v_q$. The variable $\epsilon_{pq}$, a small positive constant, reflects the navigation uncertainty and the approximation precision of the algorithm.

The overall probability of successfully navigating the entire path from $v_i$ to $v_j$, considering the sequence of edges in $P_{ij}$, is determined by the product of individual probabilities for each edge. Mathematically, this probability can be represented as $\prod_{e_{pq} \in P_{ij}} (1 - \epsilon_{pq})$, which is greater than or equal to $1 - k \max_{p,q} \epsilon_{pq}$, assuming $\epsilon = k \max_{p,q} \epsilon_{pq}$ captures the aggregated uncertainty across the path.

Therefore, the theorem confirms that TopoNav's sub-controller policy $\pi_s$ is capable of ensuring navigation between any two subgoals in the topological map with a probability of at least $1 - \epsilon$, highlighting the system's reliability in planning and executing paths under variable conditions and uncertainties. $\blacksquare$



\section{Theoretical Foundations}

\subsection{Subgoal Reachability}
\textbf{Theorem 1 (Subgoal Reachability)}. \textit{In a topological map $G = (V, E)$ designed by TopoNav, for any two nodes $v_i, v_j \in V$, there exists a high-probability path from $v_i$ to $v_j$, denoted by the sub-controller policy $\pi_s$'s capability to navigate between them with at least $1 - \epsilon$ probability, where $\epsilon$ is a small constant signifying the upper limit of navigation failure, factoring in algorithm convergence and environmental variability.}

\textbf{Proof}. Given a path $P_{ij} = \{v_i, ..., v_j\}$ comprising edges in $E$, connecting nodes in sequence from $v_i$ to $v_j$, the sub-controller policy $\pi_s$, trained via DQN principles, ensures successful navigation across each edge with probability $\geq 1 - \epsilon_{pq}$, where $\epsilon_{pq}$ is the minimal failure chance for each edge.

The cumulative success rate for the entire path $P_{ij}$, derived from sequentially navigating its edges, is calculated as $\prod_{e_{pq} \in P_{ij}} (1 - \epsilon_{pq})$. This product is bounded below by $1 - \epsilon$, with $\epsilon = k \max_{p,q} \epsilon_{pq}$ encapsulating total path uncertainty for $k$ edges.

Thus, $\pi_s$ guarantees navigation from $v_i$ to $v_j$ with probability at least $1 - \epsilon$, demonstrating TopoNav's effective pathfinding in diverse environmental conditions. $\square$

\subsection{Subgoal Generation and Navigation}
\label{subsec:subgoal_generation_navigation}

In TopoNav, subgoals are generated dynamically based on the landmarks, trees, or objects encountered by the robot while navigating towards the final goal. Whenever a new landmark or object is detected, it is compared with the existing nodes in the topological map using a similarity measure. If the similarity is below a threshold, the landmark is added as a new subgoal to the topological map.

\subsubsection{Landmark Selection Strategy}
\label{subsubsec:landmark_selection_strategy}

When multiple landmarks are detected at similar distances, TopoNav employs a selection strategy to prioritize the most informative and relevant landmark as the next subgoal. The selection criteria now include just novelty and goal-directedness.

The novelty of a landmark $l$ is calculated based on the number of previous visits, using a novelty factor that decreases exponentially with the number of visits:

\begin{equation}
N(l) = e^{-\lambda \cdot \text{visits}(l)}
\end{equation}

where $\lambda$ is a decay parameter controlling the rate at which the novelty factor decreases with visits.

The goal-directedness of a landmark is calculated as the cosine similarity between the direction vector towards the landmark and the direction vector towards the goal:

\begin{equation}
GD(l) = \frac{\mathbf{v}_l \cdot \mathbf{v}_g}{||\mathbf{v}_l|| \cdot ||\mathbf{v}_g||}
\end{equation}

where $\mathbf{v}_l$ is the direction vector towards landmark $l$, and $\mathbf{v}_g$ is the direction vector towards the goal.

The landmark selection algorithm (Algorithm \ref{alg:landmark_selection}) now calculates a score for each landmark based on a simplified combination of these criteria. The landmark with the highest score is selected as the next subgoal.

\begin{algorithm}
\caption{Landmark Selection}
\DontPrintSemicolon
\KwIn{Detected landmarks $L$, current position $\mathbf{p}$, goal position $\mathbf{g}$}
\KwOut{Selected landmark $l_{\text{best}}$}

Initialize $\text{max\_score} = -\infty$\;
\ForEach{landmark $l \in L$}{
    $N(l) = e^{-\lambda \cdot \text{visits}(l)}$\;
    $\mathbf{v}_l = \text{direction\_vector}(\mathbf{p}, l)$\;
    $\mathbf{v}_g = \text{direction\_vector}(\mathbf{p}, \mathbf{g})$\;
    $GD(l) = \frac{\mathbf{v}_l \cdot \mathbf{v}_g}{||\mathbf{v}_l|| \cdot ||\mathbf{v}_g||}$\;
    $\text{score}(l) = w_N \cdot N(l) + w_{GD} \cdot GD(l)$\;
    \If{$\text{score}(l) > \text{max\_score}$}{
        $\text{max\_score} = \text{score}(l)$\;
        $l_{\text{best}} = l$\;
    }
}
\Return $l_{\text{best}}$\;
\end{algorithm}

During navigation, the meta-controller selects the next subgoal based on the current state and the robot's overall goal. If no landmarks are detected within a certain distance threshold, TopoNav generates a new subgoal along the robot's current trajectory at the maximum detection range to ensure continuous progress towards the final goal.

The sub-controller's policy generates a sequence of primitive actions or low-level skills to navigate the robot towards the selected subgoal, aiming to maximize the expected cumulative reward. The navigation process continues until the robot reaches the subgoal or a maximum number of steps is exceeded. If the subgoal is reached, the meta-controller selects the next subgoal based on the updated state and the topological map. If the maximum number of steps is exceeded, the meta-controller selects a different subgoal or terminates the episode based on the exploration strategy.

